Weisfeiler and Leman Go Loopy: A New Hierarchy for Graph Representational Learning

We introduce $r$-loopy Weisfeiler-Leman ($r$-$\ell{}$WL), a novel hierarchy of graph isomorphism tests and a corresponding GNN framework, $r$-$\ell{}$MPNN, that can count cycles up to length $r + 2$. Most notably, we show that $r$-$\ell{}$WL can count homomorphisms of cactus graphs. This strictly extends classical 1-WL, which can only count homomorphisms of trees and, in fact, is incomparable to $k$-WL for any fixed $k$. We empirically validate the expressive and counting power of the proposed $r$-$\ell{}$MPNN on several synthetic datasets and present state-of-the-art predictive performance on various real-world datasets. The code is available at https://github.com/RPaolino/loopy

==> loopy/tabs/tudataset.tex <==
\begin{tabular}{ccccccc}
    \toprule
    & \multicolumn{6}{c}{TUDataset}\\
    \cmidrule{2-7}
    Method& DD & PROTEINS & NCI1 & ENZYMES & IMDB-B & IMDB-M \\
    \midrule
    \dgcnn{} & $76.6 \pm 4.5$ & $72.9 \pm 3.5$ & $76.4 \pm 1.7$ & $38.9 \pm 5.7$ & $69.2 \pm 3.0$ & $45.6 \pm 3.4$ \\
    \diffpool{} & $75.0 \pm 4.3$ & $73.7 \pm 3.5$ & $76.9 \pm 1.9$ & $59.5 \pm 5.6$ & $68.4 \pm 3.3$ & $45.6 \pm 3.4$ \\
    \ecc{} & $72.6 \pm 4.1$ & $72.3 \pm 3.4$ & $76.2 \pm 1.4$ & $29.5 \pm 8.2$ & $67.7 \pm 2.8$ & $43.5 \pm 3.1$ \\
    \gin{} & $75.3 \pm 2.9$ & $73.3 \pm 4.0$ & $80.0 \pm 1.4$ & $59.6 \pm 4.5$ & $71.2 \pm 3.9$ & $48.5 \pm 3.5$ \\
    \graphsage{} & $72.9 \pm 3.4$ & $70.0 \pm 4.5$ & $76.0 \pm 1.8$ & $58.2 \pm 6.0$ & $68.8 \pm 4.5$ & $47.6 \pm 3.3$ \\
    \gat{} & $73.9 \pm 3.4$ & $70.9 \pm 2.7$ & $77.3 \pm 2.5$ & $49.5 \pm 8.9$ & $69.2 \pm 4.8$ & $48.2 \pm 4.9$ \\
    \spn{}$_{\text{best}}$ & $77.4 \pm 3.8$ &$74.2 \pm 3.7$ & $80.0 \pm 1.5$ & $69.4 \pm 6.2$  & NA & NA \\
    \pathnet{} & OOM & $70.5 \pm 3.9$ & $64.1 \pm 2.3$ & $69.3 \pm 5.4$ & $70.4 \pm 3.8$ & $49.1 \pm 3.6$ \\
    \nestedgnn{} & $77.8 \pm 3.9$ & $74.2 \pm 3.7$ & NA & $31.2 \pm 6.7$ & NA & NA \\
    \pathnn{}$_{\text{best}}$ & $77.0 \pm 3.1$ & $75.2 \pm 3.9$ & $82.3 \pm 1.9$ & $73.0 \pm 5.2$ & $72.6 \pm 3.3$ & $50.8 \pm 4.5$ \\
    \midrule
    $r$-\ell{} & & \makecell{\first{$75.7\pm 3.8$}\\($r=2$)} \\
    \bottomrule
\end{tabular}




==> loopy/tabs/undistinguished.tex <==
\begin{tabular}{ccccccccc}
    \toprule
     & & Min. & 1$^\text{st}$ quartile & Median & 3$^\text{rd}$ quartile & Max & Mean & Std. \\
    \midrule
     \multirow{6}{*}{\rotatebox[origin=c]{90}{exp}} &\gnnml &  $0$ & $0$ & $0$ & $0$ & $2$ & $0.1$ & $0.33$\\
     & \ppgn{} &  $0$ & $0$ & $0$ & $1$ & $8$ & $0.55$ & $1.13$\\
     \cmidrule{2-9}
     & $r=0$ & $0$ & $0$ & $0$ & $1$ & $3$ & $0.58$ & $0.76$\\
     & $r=1$ & $0$ & $0$ & $0$ & $1$ & $3$ & $0.58$ & $0.76$\\
     & $r=2$ & $0$ & $0$ & $0$ & $1$ & $3$ & $0.58$ & $0.76$\\
     & $r=3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ &  $0$\\
     \midrule
     \multirow{6}{*}{\rotatebox[origin=c]{90}{graph8c}} &\gnnml & $0$ & $56$ & $714$ & $4\,147$ & $478\,339$  & $20\,861$ & $74\,203$ \\
     & \ppgn{} &  $287$ & $4\,434$ & $7\,718$ & $15\,292$ & $523\,646$ & $18\,120$ & $55\,024$\\
     \cmidrule{2-9}
     & $r=0$ & $994$ & $1\,557$ &   $1\,863$ &  $2\,194$ & $4\,104$ & $1\,903$ & $516$\\
     & $r=1$ & $20$ & $22$ & $24$ & $27$ & $36$ & $25$ & $4$\\
     & $r=2$ & $0$ & $0$ & $0$ & $0$ & $3$ & $0.13$ & $0.46$\\
     & $r=3$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0.04$ & $0.20$\\
     \bottomrule
\end{tabular}

==> tabs/tudataset.tex <==
\begin{tabular}{ccccccc}
    \toprule
    & \multicolumn{6}{c}{TUDataset}\\
    \cmidrule{2-7}
    Method& DD & PROTEINS & NCI1 & ENZYMES & IMDB-B & IMDB-M \\
    \midrule
    \dgcnn{} & $76.6 \pm 4.5$ & $72.9 \pm 3.5$ & $76.4 \pm 1.7$ & $38.9 \pm 5.7$ & $69.2 \pm 3.0$ & $45.6 \pm 3.4$ \\
    \diffpool{} & $75.0 \pm 4.3$ & $73.7 \pm 3.5$ & $76.9 \pm 1.9$ & $59.5 \pm 5.6$ & $68.4 \pm 3.3$ & $45.6 \pm 3.4$ \\
    \ecc{} & $72.6 \pm 4.1$ & $72.3 \pm 3.4$ & $76.2 \pm 1.4$ & $29.5 \pm 8.2$ & $67.7 \pm 2.8$ & $43.5 \pm 3.1$ \\
    \gin{} & $75.3 \pm 2.9$ & $73.3 \pm 4.0$ & $80.0 \pm 1.4$ & $59.6 \pm 4.5$ & $71.2 \pm 3.9$ & $48.5 \pm 3.5$ \\
    \graphsage{} & $72.9 \pm 3.4$ & $70.0 \pm 4.5$ & $76.0 \pm 1.8$ & $58.2 \pm 6.0$ & $68.8 \pm 4.5$ & $47.6 \pm 3.3$ \\
    \gat{} & $73.9 \pm 3.4$ & $70.9 \pm 2.7$ & $77.3 \pm 2.5$ & $49.5 \pm 8.9$ & $69.2 \pm 4.8$ & $48.2 \pm 4.9$ \\
    \spn{}$_{\text{best}}$ & $77.4 \pm 3.8$ &$74.2 \pm 3.7$ & $80.0 \pm 1.5$ & $69.4 \pm 6.2$  & NA & NA \\
    \pathnet{} & OOM & $70.5 \pm 3.9$ & $64.1 \pm 2.3$ & $69.3 \pm 5.4$ & $70.4 \pm 3.8$ & $49.1 \pm 3.6$ \\
    \nestedgnn{} & $77.8 \pm 3.9$ & $74.2 \pm 3.7$ & NA & $31.2 \pm 6.7$ & NA & NA \\
    \pathnn{}$_{\text{best}}$ & $77.0 \pm 3.1$ & $75.2 \pm 3.9$ & $82.3 \pm 1.9$ & $73.0 \pm 5.2$ & $72.6 \pm 3.3$ & $50.8 \pm 4.5$ \\
    \midrule
    $r$-\ell{} & & \makecell{\first{$75.7\pm 3.8$}\\($r=2$)} \\
    \bottomrule
\end{tabular}




==> tabs/undistinguished.tex <==
\begin{tabular}{ccccccccc}
    \toprule
     & & Min. & 1$^\text{st}$ quartile & Median & 3$^\text{rd}$ quartile & Max & Mean & Std. \\
    \midrule
     \multirow{6}{*}{\rotatebox[origin=c]{90}{exp}} &\gnnml &  $0$ & $0$ & $0$ & $0$ & $2$ & $0.1$ & $0.33$\\
     & \ppgn{} &  $0$ & $0$ & $0$ & $1$ & $8$ & $0.55$ & $1.13$\\
     \cmidrule{2-9}
     & $r=0$ & $0$ & $0$ & $0$ & $1$ & $3$ & $0.58$ & $0.76$\\
     & $r=1$ & $0$ & $0$ & $0$ & $1$ & $3$ & $0.58$ & $0.76$\\
     & $r=2$ & $0$ & $0$ & $0$ & $1$ & $3$ & $0.58$ & $0.76$\\
     & $r=3$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ &  $0$\\
     \midrule
     \multirow{6}{*}{\rotatebox[origin=c]{90}{graph8c}} &\gnnml & $0$ & $56$ & $714$ & $4\,147$ & $478\,339$  & $20\,861$ & $74\,203$ \\
     & \ppgn{} &  $287$ & $4\,434$ & $7\,718$ & $15\,292$ & $523\,646$ & $18\,120$ & $55\,024$\\
     \cmidrule{2-9}
     & $r=0$ & $994$ & $1\,557$ &   $1\,863$ &  $2\,194$ & $4\,104$ & $1\,903$ & $516$\\
     & $r=1$ & $20$ & $22$ & $24$ & $27$ & $36$ & $25$ & $4$\\
     & $r=2$ & $0$ & $0$ & $0$ & $0$ & $3$ & $0.13$ & $0.46$\\
     & $r=3$ & $0$ & $0$ & $0$ & $0$ & $1$ & $0.04$ & $0.20$\\
     \bottomrule
\end{tabular}
